Discriminatory or Samaritan -- which AI is needed for humanity? An Evolutionary Game Theory Analysis of Hybrid Human-AI populations

As artificial intelligence (AI) systems are increasingly embedded in our lives, their presence leads to interactions that shape our behaviour, decision-making, and social interactions. Existing theoretical research has primarily focused on human-to-human interactions, overlooking the unique dynamics triggered by the presence of AI. In this paper, resorting to methods from evolutionary game theory, we study how different forms of AI influence the evolution of cooperation in a human population playing the one-shot Prisoner's Dilemma game in both well-mixed and structured populations. We found that Samaritan AI agents that help everyone unconditionally, including defectors, can promote higher levels of cooperation in humans than Discriminatory AI that only help those considered worthy/cooperative, especially in slow-moving societies where change is viewed with caution or resistance (small intensities of selection). Intuitively, in fast-moving societies (high intensities of selection), Discriminatory AIs promote higher levels of cooperation than Samaritan AIs.

==> sections/literature_review.tex <==
\section{Literature Review}

\subsection{Prisoner's Dilemma}
The original version of the Prisoner’s Dilemma is a two-person, symmetrical non-zero sum game and was first conceptualized by Merrill Flood and Melvin Dresher (1950) and expanded by Albert William Tucker (1950). The players are rational and have the choice between two strategies, to cooperate with or betray the other player. Their goal is the maximization of their payoffs, not knowing anything about the opponent’s course of action \citep{rios2015prisoner}. 
If both players choose to cooperate, they receive a reward (R), and if both defect they will receive a punishment (P). When the cooperator meets a defector, she will receive S and the defector gets T. T > R > P > S and 2R>T+S. \citep{xianyu2012prisoner} 
Given this payoff matrix and model version, mutual defection is the dominant strategy for the players from the perspective of individual rationality. Yet, cooperation would yield the maximum payoff overall \citep{rios2015prisoner}. 
In 1973, the mathematical biologists John Maynard Smith and George Price published “The logic of animal conflict” considered to be the birth of evolutionary game theory \citep{smith1973logic}. The focus in evolutionary game theory lies with the dynamics of strategy change in a population of agents facilitated by social learning strategies via selection and mutation \citep{chong2007}. What drives the dynamics is not the rationality of the players but rather the difference in the payoffs yielded by the strategies of players in an interaction. 
In evolutionary game theory, the prisoner’s dilemma is used to study the evolution of cooperation and defection strategies over time. The strategy phenotypes have a fitness that is denoted by the payoffs. The higher the fitness, the greater the reproductive success and spreading of the strategy in large populations over time. \citep{rios2015}

phenomenon depends on the selection pressure, update rule, and network structure in other types of games. 

Resolution of the social dilemma: Positive assortativity
What alterations to the original model can facilitate the survival of a cooperative regime?
In general, according to research on cooperative AI by \citep{dafoe2020open}, the cooperative equilibrium can be achieved via mechanisms that create a conditional commitment, communication or the ability to predict other players' behavior. For example, commitments can be implemented by repeated play, the costs of one’s reputation, a contract or a physical constraint \cite {dafoe2020open}. Another method is to ‘change the game’ which can be achieved by the creation of institutions. These institutions are effective in facilitating collective cooperation, if they promote cooperative understanding, communication or commitments. What all of these methods share, is the mutual identification of cooperating players, called positive assortativity \citep{pepper2002mechanism}.

In the case of a one-shot game with no memory and reputation mechanisms, positive assortativity is not possible. The cooperative regime can be achieved nonetheless by way of rewarding altruists, the optional PD, where players can also opt-out, punishing defectors, as well as the introduction of zealot players \citep{sharma2023small}.  
The last two options will be sketched out in more detail.
The punishment of defectors can be achieved by way of third party punishment or altruistic punishment. According to \citep{fehr2004third}, third party punishment is directly related to the enforcement of norms that regulate human behavior. If a first party, or defector, harms a second party, or cheated player, we can introduce a third party that is unaffected by the violation and who can impose a punishment on the norm violating player. The action, however, is costly for the third party and does not incur a reward. For a rational agent, it would be illogical to engage in punishing the first party at a personal cost. In other words, the third party punishment presents a dilemma of social cooperation \citep{fehr2004third}. 
In the case of our model, however, the third party is played by an AI, that does not bear the cost of punishment and effectively solves the dilemma. 
Contrary to basic tenets of evolutionary game theory, zealous players are a type of agent that does not imitate other players' strategy but remains committed regardless of payoffs \citep{nakajima2015evolutionary}. The mechanism that shifts the equilibrium of defectors towards cooperation with a certain number of zealous cooperators, is the increased probability cooperative individuals to encounter other cooperators. However, according to this effect can only be observed in well-mixed populations \citep{sharma2023small}. 

In a recent theoretical study on the impact of human-bot interactions on the evolution of cooperation by \citep{sharma2023small}, the authors model the cooperative  bots as zealous agents under the name "committed individuals". The study models four types of bots in an optional prisoners dilemma game. The strategies available are defection, cooperation and what they term 'loner' or the opt-out action. The first AI always chooses to cooperate, the second version, always chooses to defect, the third AI bot always chooses to opt-out and the fourth type is designed to choose the three strategies with equal likelihood. Each of these bots will run on two types of population structures: a well-mixed population, meaning an equal probability to interact and a square lattice, only allowing for interaction with their nearest neighbors.

They found that in the well-mixed and square lattice population model, with a low imitation parameter resolved the collective cooperation problem. The loner bots could shift the equilibrium towards cooperation in the square lattice under a strong imitation assumption but only below a threshold number of the AI agents. The experiment confirms their hypothesis that even in cooperation adverse conditions such as the one-shot, anonymous, well-mixed Prisoner's Dilemma, cooperation regimes can become dominant through the strategic deployment of zealous AI cooperators \citep{sharma2023small}. 

\subsection{Human Strategic Decision-Making in Hybrid-AI Systems}
While research on strategic decision-making in the presence of autonomous intelligent agents is relatively scarce, hybrid-AI interactions have been investigated since the 1970s in the field of economic behavior. 
Early research was conducted on the use of computer players in economic behavioral experiments. March et al. (2015)’s extensive review of 90 such experimental studies reveals concludes that human agents act more selfishly and at the same time more rational in strategic interactions with autonomous agents. Moreover, a study by \citep{cohn2022honesty} found that human players tend to exploit the autonomous agents by cheating and distinctly dishonest human players prefer to play with autonomous agents for this reason \citep{fernandez2022delegation}. So the dominant strategy towards autonomous intelligent agents is less likely to be cooperative than towards human players. This discriminatory effect can be partly reversed by humanizing the AI agent "in visual, emotional and cultural cues" demonstrated in an experimental study by \citep{de2019cooperation}. Especially the implementation of emotional cues may be effective at re-aligning the cooperation propensity to human-on-human interaction levels. 
As articulated in \citep{fernandez2022delegation}, some research has yielded that emotional cues may shape how humans designate reputations to other agents. This seems to point towards an underlying trust factor in human strategic interactions, especially relevant in human-AI interactions.
A paper by \citep{han2021or} argues that trust-based strategies are employed by human agents to avoid using computationally costly conditional strategies to infer the predictability of another player's cooperative behavior in repeated games \citep{han2021or}. As human agents only have partial information of the autonomous intelligent agents, the cost of predicting the intelligent autonomous agent's cooperative strategy is especially costly and this would suggest that humans would be more likely to use trust-based strategies in human-AI interactions. In other words, the role of trust in human-AI interactions should be greater than in human-to-human interactions \citep{han2021or}.

